PS-EIP: Robust Photometric Stereo Based on Event Interval Profile

Recently, the energy-efficient photometric stereo method using an event camera has been proposed to recover surface normals from events triggered by changes in logarithmic Lambertian reflections under a moving directional light source. However, EventPS treats each event interval independently, making it sensitive to noise, shadows, and non-Lambertian reflections. This paper proposes Photometric Stereo based on Event Interval Profile (PS-EIP), a robust method that recovers pixelwise surface normals from a time-series profile of event intervals. By exploiting the continuity of the profile and introducing an outlier detection method based on profile shape, our approach enhances robustness against outliers from shadows and specular reflections. Experiments using real event data from 3D-printed objects demonstrate that PS-EIP significantly improves robustness to outliers compared to EventPS's deep-learning variant, EventPS-FCN, without relying on deep learning.

==> outline/o3_preliminaries.tex <==
\section{Preliminaries}



\subsection{Mechanism of event camera}
event generation

\subsection{Pixel circuit signals of event camera}
画素回路の構成要素:
    photoreceptor, logarithmic amplifier, and differentiator.\\
各出力信号: \cite{}$\sigp$, $\siga$, $\sigd$.
\begin{equation}
    \sigp = \radiance
\end{equation}
\begin{equation}
    \siga = \ln{\sigp}
\end{equation}
\begin{equation}
    \sigd = \ddt{\siga}
\end{equation}
Then
\begin{equation}
    \sigd = \frac{\ddt{\radiance}}{\radiance}
\end{equation}
$\sigd$は$\radiance$の対数微分になる



==> outline/o4_method.tex <==
\section{Proposed method}
\label{sec:method}



\subsection{Radiance of Lambertian surface}
radiance (Lambertian case):\\
\begin{equation}
    \radiance = \source \albedo \nldot
\end{equation}
rewrite $\normal$ and $\lightvec$ in spherical coordinate system
\begin{equation}
    \normal = 
        \begin{bmatrix}
            \sin{\theta_n} \cos{\phi_n}\\
            \sin{\theta_n} \sin{\phi_n}\\
            \cos{\theta_n}\\
        \end{bmatrix},
    \lightvec = 
        \begin{bmatrix}
            \sin{\theta_l} \cos{\phi_l}\\
            \sin{\theta_l} \sin{\phi_l}\\
            \cos{\theta_l}\\
        \end{bmatrix}
\end{equation}
Then
\begin{equation}
    \nldot = \sin{\theta_n} \sin{\theta_l} \cos{(\phi_l - \phi_n)} + \cos{\theta_n} \cos{\theta_l} \\
\end{equation}

\subsection{Rotating light}
光源方向がカメラ光軸で回転.
\begin{equation}
    \theta_l = \const, 
    \phi_l = a t + b % 線形関数
\end{equation}
定数になる部分を、簡単のためA,Bで書き換える
\begin{equation}
    A = \sin{\theta_n} \sin{\theta_l},
    B = \cos{\theta_n} \cos{\theta_l}
\end{equation}
輝度:
\begin{equation}
    \radiance = \source \albedo (A \cos{(\phi_l - \phi_n)} + B)
\end{equation}
輝度の対数微分:
\begin{equation}
    \frac{\ddt{\radiance}}{\radiance} = \frac{-A \sin{(\phi_l - \phi_n)}}{A \cos{(\phi_l - \phi_n)} + B} \ddt{\phi_l}
\end{equation}

\subsection{$\dt$ and $\sigd$}
各イベント時刻の$\sigd$を近似する。 \\
\begin{equation}
    \sigd(t_n) \simeq \frac{\siga(t_{n}) - \siga(t_{n-1})}{t_{n} - t_{n-1}} = \frac{\thresh}{\dt_{n-1,n}}
\end{equation}
$\thresh$: 閾値 \\
$\dt$: イベント間隔 \\
$t_n$: イベント時刻 \\
より良い結果のために次の定義を使った（実装）
\begin{equation}
    \sigd(t_n) \simeq \frac{\siga(t_{n+1}) - \siga(t_{n-1})}{t_{n+1} - t_{n-1}} = \frac{2 \thresh}{\dt_{n-1,n} + \dt_{n,n+1}}
\end{equation}
これは前後の$\frac{\thresh}{\dt}$の$\dt$での重み付き和になっている

\subsection{Fitting}
profileを定義 \\
$t \in [0,period)$での輝度の対数微分
\begin{equation}
    \profile = \sigd(t)
\end{equation}
$period$ は周期\\
Profileは$\normal (\phi_n, \theta_n)$から計算できる\\
\begin{equation}
    \profile_{sim} =\sigd(\phi_l, \phi_n, \theta_n)
\end{equation}
Profileはイベント列から復元できる
各イベントの$\sigd(t_n)$を線形補間する\\
等間隔でサンプリングしたベクトルをprofileとして使う\\
\begin{equation}
    \profile_{obs} = \lerp{\sigd(t_n)}
\end{equation}
２つのprofileのerrorをMSEで計算\\
maskされた部分は使わない
\begin{equation}
    error = \mse{\profile_{sim}, \profile_{obs}}
\end{equation}
コスト関数を定義 \\
探索パラメータは$\normal$
\begin{equation}
    \cost{\normal | \profile_{obs}} = \mse{\profile_{sim}(\normal), \profile_{obs}}
\end{equation}

\begin{equation}
    minimize: \cost{\normal | \profile_{obs}}
\end{equation}

\subsection{ambient light}
影では $\radiance=0$.\\
$\siga = \ln{0}$ は未定義なので不適切\\
ambient light によって $\radiance$ が小さくならないようにする.\\
$\normal$ が定まったとき、 $ \amb{\normal}$ も定まる必要がある\\
$\source$に対する$\ambs$の比$\frac{\ambs}{\source}$は既知とする. \\
$\albedo$ is surface albedo. \\
$\source$ is rotating light strength.\\
$\ambs$ is ambient light strength.
\begin{enumerate}
    \item $\nldot > 0$の場合:
        \begin{align}
            \radiance &= \source \albedo (\nldot) + \ambs \albedo (\amb{\normal}) \\
            &= \source \albedo (A \cos{(\phi_l - \phi_n)} + B + \frac{\ambs}{\source} \amb{\normal}) \\
            \ddt{\radiance} &= \source \albedo (-A \sin{(\phi_l - \phi_n)}) \ddt{\phi_l} \\
            \sigd &= \frac{-A \sin{(\phi_l - \phi_n)}}{A \cos{(\phi_l - \phi_n)} + B + \frac{\ambs}{\source}\amb{\normal}} \ddt{\phi_l}
        \end{align}
    \item $\nldot\ \leq 0$の場合:
        \begin{align}
            \radiance &= \ambs \albedo (\amb{\normal}) \\
            \ddt{\radiance} &= 0 \\
            \sigd &= 0
        \end{align}
\end{enumerate}

\subsection{highlight and cast shadow}
mask


==> outline/o5_experiments.tex <==
\section{Experiments}
\label{sec:intro}

\subsection{Setup}
\subsubsection{light}
LED ring light \\
光量を線形補間 \\
lpfでpwmの影響を除く \\
\subsubsection{ambient light}
全LEDを弱く点灯させ、これをambient lightとする。 \\
このambient lightによる輝度は、単光源輝度のリングライトに沿っての積分である。\\
attached shadow の有無によって$\amb{\normal}$の算出法が変わる \\
まず、$\nldot = A \cos{(\phi_l - \phi_n)} + B$であるから、
\begin{align}
    \min_{\phi_l \in [0,2\pi]}{(\nldot)} &= -A+B
\end{align}
\begin{enumerate}
    \item $\min{(\nldot)} > 0$の場合: \\
        光源が回転しても常に照らされている
        \begin{align}
            \amb{\normal} &= \int_0^{2\pi}{ (A \cos{(\phi_l - \phi_n)} + B) d\phi_l} \\
                            &= 2 \pi B
        \end{align}
    \item $\min{(\nldot)} \leq 0$の場合: \\
        attached shadow になる$\phi_l$の区間が存在する \\
        光が当たる条件は$ A \cos{(\phi_l - \phi_n)} + B > 0 $だから、
        光が当たる$\phi_l$の区間は
        \begin{align}
            \phi_n - C  < \phi_l < \phi_n + C \\
            C = \arccos{(-B/A)}
        \end{align}
        よってこれを積分範囲として
        \begin{align}
            \amb{\normal} &= \int_{\phi_n - C}^{\phi_n + C}{ (A \cos{(\phi_l - \phi_n)} + B) d\phi_l} \\
                            &= 2 \int_{0}^{C}{ (A \cos{(\phi)} + B) d\phi} \\
                            &= 2 ( A \sin{C} + B C )
        \end{align}
\end{enumerate}

\subsection{exp1}
\subsubsection{lambertian}
\subsubsection{lambertian with albedo}
\subsubsection{highlight}
\subsubsection{cast shadow}
\subsubsection{difficult case}

\subsection{exp2}
\subsubsection{3d printed data}
\subsubsection{realistic object} 

==> outline/o9_Implemantation.tex <==
\section{Implemantation}
\label{sec:intro}

\subsection{光源変調}
離散的に配置された光源の変調で、連続的な光源移動による輝度変化を模倣 \\
隣り合う光源の光量を線形に変調する \\
\begin{itemize}
    \item はじめ、光源nが最大光量で、他は最小とする。\\
    \item 光量の総和を保ちながら、光源nの光量を線形に下げ、光源n+1の光量を線形に上げる。\\
    \item 光源nが最小光量になり、n+1が最大光量になる。\\
\end{itemize}
実際の値の例 \\  
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \hline
    led0 & 241 & 161 & 81 & 1 & 1 & 1 & 1 & 1 & 1 \\
    \hline
    led1 & 1 & 81 & 161 & 241 & 161 & 81 & 1 & 1 & 1 \\
    \hline
    led2 & 1 & 1 & 1 & 1 & 81 & 161 & 241 & 161 & 81 \\
    \hline
    led3 & 1 & 1 & 1 & 1 & 1 & 1 & 1 & 81 & 161 \\
    \hline
\end{tabular}
\begin{itemize}
    \item ledの光量が、ステップごとにどのような値を取るか
    \item １ステップごとに光量が80ずつ変化 3ステップで最大光量に
    \item オフセットとして１が加算されている
    \item １週およそ0.8sほど
\end{itemize}

\subsection{閾値計測}
正イベントのみを考える。 \\
輝度 \radiance は \time に対して単調に増加するとする。 \\
まず、時刻 $\time_0$ と $\time_1$ でイベントが発生したとする。 \\
これに対し、閾値 \thresh を次のように定義する。
\begin{align}
    \ln{\radiance[\time_1]} - \ln{\radiance[\time_0]} 
    = \ln{\frac{\radiance[\time_1]}{\radiance[\time_0]}}
    = \thresh
\end{align}
つづいて、時刻 $\time_0$ から $\time_1$ までにイベントが \evnum 回発生したとする。 \\
このとき次式が成り立つ。 \\
\begin{align}
    \ln{\radiance[\time_1]} - \ln{\radiance[\time_0]} 
    = \ln{\frac{\radiance[\time_1]}{\radiance[\time_0]}}
    \simeq \thresh \evnum
\end{align}
イベントカメラ、物体、光源があるシーンを考える。 \\
\begin{align}
    \radiance[\time] = \source(\time) \brdf \\
\end{align}{}
時刻 $\time_0$ から $\time_1$ で、光源光量のみを変化した場合、
\brdf は定数であるから、 \\
\begin{align}
    \ln{\frac{\radiance[\time_1]}{\radiance[\time_0]}} 
    &= \ln{\frac{\source(\time_1) \brdf}{\source(\time_0) \brdf}} \\
    &= \ln{\frac{\source(\time_1)}{\source(\time_0)}}
\end{align}
時刻 $\time_0$ から $\time_1$ で光源光量を $k$ 倍に変化させたときに、イベントが \evnum 回発生したとする。
このとき次式によって \thresh が求められる。 \\
\begin{align}
    \thresh \simeq \frac{\ln{k}}{\evnum}
\end{align}
実際の計測では、LED光源を3つ使い、 $k = 6$ として光源変調をした。\\
 c 回光源を明滅させる。$(c \simeq 40)$ \\
発生イベントの総数を $\evnum_{pos}, \evnum_{neg}$ とする \\
\begin{align}
    \thresh_{pos} &= \frac{\ln{k}}{\evnum_{pos} c} \\
    \thresh_{neg} &= \frac{\ln{k}}{\evnum_{neg} c}
\end{align}
一般に、$\ln{\frac{\radiance[\time_1]}{\radiance[\time_0]}}$ は \thresh の整数倍でないので、何度も計測しても正確な \thresh を求められるわけではない。 \\
$c$ が十分大きければ、それらしい結果を得られている。（比較検証はしていない） \\
$k=6$ の場合、 \evnum は 10--20 ほどだった（多分）\\

\subsection{プロファイル生成}
イベントごとに、前後のイベントとの時刻差の平均を算出して \dt とする \\
極性に基づいた \thresh とともに、 $\frac{\thresh}{\dt}$ を計算 \\
各イベントの \time と $\frac{\thresh}{\dt}$ を線形補間した関数を定数長でサンプリング \\
処理時に最初と最後の周期は使わない。30周期からプロファイルを作るなら32周期分のデータを使う


==> outline/ox_figs.tex <==
\section{figs}

\begin{figure}[t]
    
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs_supp/shape/prof_azi.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs_supp/shape/prof_zen.pdf}
    \end{subfigure}

    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs_supp/margin/margin_gloss.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs_supp/margin/margin_cast.pdf}
    \end{subfigure}

    \begin{subfigure}[t]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figs_supp/log/img_patches.pdf}
    \end{subfigure}

\end{figure}

==> sec/Z6a_eval_spheres.tex <==
\begin{figure}[t]
    % Settings
    \newcommand{\cellwidth}{0.185\linewidth} % 11.390
    % \newcommand{\colorbarwidth}{0.023125\linewidth} % 0.185 / 8
    % \newcommand{\colorbarwidth}{0.0115\linewidth} % 0.185 / 16
    \newcommand{\colorbarwidth}{0.038\linewidth} % 0.185 / 16
    \newcommand{\cellheight}{\linewidth}
    \setlength\tabcolsep{0pt}
    \footnotesize
    \centering
        
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccccccc}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & Photo & \heatmap & Recovery & GT & AE \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\diffusesphere} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/diffusesphere.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_diffuse/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_diffuse/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_diffuse/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/sphere_diffuse/ang_error.jpg}}
                \put(3,3){\mae{2.91}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\glossysphere} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/specularsphere.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_gloss/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_gloss/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_gloss/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/sphere_gloss/ang_error.jpg}}
                \put(3,3){\mae{3.16}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\shadowsphere} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/castsphere.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_cast/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_cast/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_cast/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/sphere_cast/ang_error.jpg}}
                \put(3,3){\mae{3.84}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\twocolorsphere} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/2colorsphere.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_diffuse/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_diffuse/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_diffuse/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/sphere_albedo2_diffuse/ang_error.jpg}}
                \put(3,3){\mae{3.38}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\multirefsphere} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/multirefsphere.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_multi/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_multi/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_multi/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/sphere_albedo2_multi/ang_error.jpg}}
                \put(3,3){\mae{3.30}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \end{tabular*}
    
    \caption{Quantitative evaluation with the sphere-based shapes. From left to right: photograph, event accumulation image from the events, recovered normal map, ground truth, and angular error map.}
    \label{fig:eval spheres}
\end{figure}


==> sec/Z6b_eval_complicated.tex <==
\begin{figure}[t]
    % Settings
    \newcommand{\cellwidth}{0.185\linewidth}
    \newcommand{\colorbarwidth}{0.038\linewidth}
    \newcommand{\cellheight}{\linewidth}
    \setlength\tabcolsep{0pt}
    \footnotesize
    \centering

    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccccccc}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & Photo & \heatmap & Recovery & GT & AE \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\bunny} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/bunny.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/bunny/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/bunny/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/bunny/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/bunny/ang_error.jpg}}
                \put(3,3){\mae{12.0}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}             
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\caesar} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/head.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/germnicus/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/germnicus/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/germnicus/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/germnicus/ang_error.jpg}}
                \put(3,3){\mae{9.35}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}             
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\baboon} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/baboon.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/baboon/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/baboon/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/baboon/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/baboon/ang_error.jpg}}
                \put(3,3){\mae{8.80}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}             
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \rotatebox[origin=l]{90}{\cube} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \centering
        %     \includegraphics[height=\cellheight]{figs/obj/cube.jpg}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \centering
        %     \includegraphics[height=\cellheight]{figs/results/cube/heatmap.jpg}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \centering
        %     \includegraphics[height=\cellheight]{figs/results/cube/normals_obs.jpg}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \centering
        %     \includegraphics[height=\cellheight]{figs/results/cube/normals_ref.jpg}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \begin{picture}(\cellwidth, \cellheight)
        %         \put(0,0){\includegraphics[height=\cellheight]{figs/results/cube/ang_error.jpg}}
        %         \put(3,3){\mae{6.96}}
        %     \end{picture}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\colorbarwidth}             
        %     \centering
        %     \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        % \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\cv} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/cv.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/cv/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/cv/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/cv/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/cv/ang_error.jpg}}
                \put(3,3){\mae{6.99}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}             
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % \rotatebox[origin=l]{90}{\brick} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \centering
        %     \includegraphics[height=\cellheight]{figs/obj/brick.jpg}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \centering
        %     \includegraphics[height=\cellheight]{figs/results/brick/heatmap.jpg}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \centering
        %     \includegraphics[height=\cellheight]{figs/results/brick/normals_obs.jpg}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \centering
        %     \includegraphics[height=\cellheight]{figs/results/brick/normals_ref.jpg}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\cellwidth}
        %     \begin{picture}(\cellwidth, \cellheight)
        %         \put(0,0){\includegraphics[height=\cellheight]{figs/results/brick/ang_error.jpg}}
        %         \put(3,3){\mae{10.05}}
        %     \end{picture}
        % \end{subfigure} &
        % \begin{subfigure}[t]{\colorbarwidth}             
        %     \centering
        %     \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        % \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\floral} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/floral.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/floral/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/floral/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/floral/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/floral/ang_error.jpg}}
                \put(3,3){\mae{15.86}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}             
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    \end{tabular*}
    
    \caption{Quantitative evaluation with the complicated shapes. From left to right: photograph, event accumulation image from the events, recovered normal map, ground truth, and angular error map.}
    \label{fig:eval complicated}
\end{figure}


==> sec/Z6c_eval_practical.tex <==
\begin{figure}[t]
    % Settings
    \newcommand{\cellwidth}{0.19\linewidth}
    \newcommand{\cellheight}{\linewidth}
    \setlength\tabcolsep{0pt}
    \footnotesize
    \centering

    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cccccc}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & Photo & \heatmap & Recovery & \multicolumn{2}{c}{Depth} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\miffy} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/miffy.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/miffy_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/miffy_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/miffy_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/miffy_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\retriever} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/retriever.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/garden_dog1_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/garden_dog1_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/garden_dog1_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/garden_dog1_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\cactusA} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/cactus3.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/cactus3_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/cactus3_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/cactus3_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/cactus3_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\medalcat} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/medal_cat.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/medal_cat_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/medal_cat_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/medal_cat_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/medal_cat_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        
    
    \end{tabular*}
    
    \caption{
    Qualitative evaluation with the practical objects. From left to right: photograph, event accumulation image from events, recovered normal map, and depth from the normal map.}
    \label{fig:eval practical}
\end{figure}




==> sec/ZXa_eval_printed.tex <==
\begin{figure}[t]
    % Settings
    \newcommand{\cellwidth}{0.185\linewidth} % 11.390
    % \newcommand{\colorbarwidth}{0.023125\linewidth} % 0.185 / 8
    % \newcommand{\colorbarwidth}{0.0115\linewidth} % 0.185 / 16
    \newcommand{\colorbarwidth}{0.038\linewidth} % 0.185 / 16
    \newcommand{\cellheight}{\linewidth}
    \setlength\tabcolsep{0pt}
    \footnotesize
    \centering
        
    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}ccccccc}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & Photo & \heatmap & Recovery & GT & AE \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\twocolorglossysphere} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/specular2colorsphere.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_gloss/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_gloss/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo2_gloss/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/sphere_albedo2_gloss/ang_error.jpg}}
                \put(3,3){\mae{3.48}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\diffuseyr} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/obj/sphere_diffuse4.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo3_diffuse/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo3_diffuse/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_albedo3_diffuse/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/sphere_albedo3_diffuse/ang_error.jpg}}
                \put(3,3){\mae{3.79}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\diffusebg} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/obj/sphere_albedo_bg.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_albedo_bg_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_albedo_bg_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_albedo_bg_normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_albedo_bg_ang_error.jpg}}
                \put(3,3){\mae{5.02}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\semiglossy} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/obj/sphere_semigloss.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_semigloss_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_semigloss_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_semigloss_normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_semigloss_ang_error.jpg}}
                \put(3,3){\mae{3.43}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\cube} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/cube.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/cube/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/cube/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/cube/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/cube/ang_error.jpg}}
                \put(3,3){\mae{6.96}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\brick} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/brick.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/brick/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/brick/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/brick/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/brick/ang_error.jpg}}
                \put(3,3){\mae{10.05}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\glossycv} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/obj/cv_gloss.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/cv_gloss3_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/cv_gloss3_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/cv_gloss3_normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs_supp/results_printed/cv_gloss3_ang_error.jpg}}
                \put(3,3){\mae{7.24}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\multirefsbunny} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/obj/bunny_multi.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/bunny_multi_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/bunny_multi_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/bunny_multi_normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs_supp/results_printed/bunny_multi_ang_error.jpg}}
                \put(3,3){\mae{12.43}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\twopoles} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj/castsphere2.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_cast_double/heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_cast_double/normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results/sphere_cast_double/normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs/results/sphere_cast_double/ang_error.jpg}}
                \put(3,3){\mae{5.98}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\blacksphere} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/obj/sphere_black.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_black_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_black_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_black_normals_ref.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \begin{picture}(\cellwidth, \cellheight)
                \put(0,0){\includegraphics[height=\cellheight]{figs_supp/results_printed/sphere_black_ang_error.jpg}}
                \put(3,3){\mae{35.77}}
            \end{picture}
        \end{subfigure} &
        \begin{subfigure}[t]{\colorbarwidth}
            \centering
            \includegraphics[width=\linewidth]{figs/results/colorbar1.pdf}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
    \end{tabular*}
    
    \caption{Additional, quantitative evaluation with 3D printed objects. From left to right: photograph, event accumulation image from the events, recovered normal map, ground truth, and angular error map.}
    \label{fig:additional eval printed}
\end{figure}


==> sec/ZXb_eval_practical.tex <==
\begin{figure}[t]
    % Settings
    \newcommand{\cellwidth}{0.19\linewidth}
    \newcommand{\cellheight}{\linewidth}
    \setlength\tabcolsep{0pt}
    \footnotesize
    \centering

    \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}cccccc}
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        & Photo & \heatmap & Recovery & \multicolumn{2}{c}{Depth} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\owl} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/owl.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/owl_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/owl_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/owl_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/owl_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\whitedog} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/white_frenchbulldog.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/white_dog_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/white_dog_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/white_dog_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/white_dog_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\satwhitedog} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/white_frenchbulldog_sit.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/white_dog2_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/white_dog2_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/white_dog2_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/white_dog2_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\cactusB} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/cactus1.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/cactus1_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/cactus1_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/cactus1_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/cactus1_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\cactusC} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/cactus2.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/cactus2_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/cactus2_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/cactus2_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/cactus2_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\elmo} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/elmo.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/elmo_front_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/elmo_front_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/elmo_front_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/elmo_front_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\bear} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/bear.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/bear_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/bear_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/bear_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/bear_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\panda} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/panda.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/panda_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/panda_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/panda_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/panda_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\rody} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/rody.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/rody_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/rody_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/rody_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/rody_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\soccerfrog} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/soccer_frog.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/football_frog_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/football_frog_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/football_frog_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/football_frog_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\tenniscat} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/tennis_cat.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/tennis_cat_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/tennis_cat_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/tennis_cat_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/tennis_cat_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \rotatebox[origin=l]{90}{\medalfrog} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/obj_real/medal_frog.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/medal_frog_heatmap.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]            {figs/results_real/medal_frog_normals_obs.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight]{figs/results_real/medal_frog_depth.jpg}
        \end{subfigure} &
        \begin{subfigure}[t]{\cellwidth}
            \centering
            \includegraphics[height=\cellheight] {figs/results_real/angle2/medal_frog_depth.jpg}
        \end{subfigure} \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    \end{tabular*}
    
    \caption{
    Additional, qualitative evaluation with the practical objects. From left to right: photograph, event accumulation image from events, recovered normal map, and depth from the normal map.}
    \label{fig:additional eval practical}
\end{figure}
